Sparse Coding with Fast Image Alignment via Large Displacement Optical Flow

Sparse representation-based classifiers have shown outstanding accuracy and robustness in image classification tasks even with the presence of intense noise and occlusion. However, it has been discovered that the performance degrades significantly either when test image is not aligned with the dictionary atoms or the dictionary atoms themselves are not aligned with each other, in which cases the sparse linear representation assumption fails. In this paper, having both training and test images misaligned, we introduce a novel sparse coding framework that is able to efficiently adapt the dictionary atoms to the test image via large displacement optical flow. In the proposed algorithm, every dictionary atom is automatically aligned with the input image and the sparse code is then recovered using the adapted dictionary atoms. A corresponding supervised dictionary learning algorithm is also developed for the proposed framework. Experimental results on digit datasets recognition verify the efficacy and robustness of the proposed algorithm.

==> Makefile <==
FILENAME = icip_paper
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf

# PAPERSIZE = a4
PAPERSIZE = letter

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE)
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . Tables Figures
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:
	latex main
	@if grep "Warning: Citation" main.log; then bibtex main; \
	latex main; fi;
	@while grep Rerun main.log; do latex main; done;

ps: main
	dvips -t $(PAPERSIZE) -o $(PS_FILE) main

pdf: main
	dvips -t $(PAPERSIZE) -Ppdf -j0 -G0 -o $(PS_FILE) main
	ps2pdf -sPAPERSIZE=$(PAPERSIZE) \
		-dPDFSETTINGS=/prepress \
		-dCompatibilityLevel=1.7 \
		$(PS_FILE) $(PDF_FILE)

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done

